Are AlphaZero-like Agents Robust to Adversarial Perturbations?

The success of AlphaZero (AZ) has demonstrated that neural-network-based Go AIs can surpass human performance by a large margin. Given that the state space of Go is extremely large and a human player can play the game from any legal state, we ask whether adversarial states exist for Go AIs that may lead them to play surprisingly wrong actions. In this paper, we first extend the concept of adversarial examples to the game of Go: we generate perturbed states that are ``semantically'' equivalent to the original state by adding meaningless moves to the game, and an adversarial state is a perturbed state leading to an undoubtedly inferior action that is obvious even for Go beginners. However, searching the adversarial state is challenging due to the large, discrete, and non-differentiable search space. To tackle this challenge, we develop the first adversarial attack on Go AIs that can efficiently search for adversarial states by strategically reducing the search space. This method can also be extended to other board games such as NoGo. Experimentally, we show that the actions taken by both Policy-Value neural network (PV-NN) and Monte Carlo tree search (MCTS) can be misled by adding one or two meaningless stones; for example, on 58\% of the AlphaGo Zero self-play games, our method can make the widely used KataGo agent with 50 simulations of MCTS plays a losing action by adding two meaningless stones. We additionally evaluated the adversarial examples found by our algorithm with amateur human Go players and 90\% of examples indeed lead the Go agent to play an obviously inferior action. Our code is available at \url{https://PaperCode.cc/GoAttack}.

==> algorithm.tex <==


\subsection{Proposed Algorithm}

Like other adversarial attack on reinforcement learning, we attack an agent with a game instead of just one state. That is, given a game $G = \{s_0, s_1, \dots, s_T\}$, if we can find one pair of $(s_i, s_i')$, where $s_i'$ is an adversarial example of $s_i$, then we have successfully attack the agent on that game. 
We do not ask our algorithm to successfully attack every state of the game since it only takes one mistake for an agent to lose a game. Another benefit of attacking all the states of a same game is that the searching result of one state can be used to accelerate the searching process of other states.

Given a game, our algorithm will first apply the 1STEP attack. If the 1STEP attack fails, we will then  apply the 2STEP attack. Since the search space is countable, we can brute force check all the states in the search space. However, the time complexity is too high. For example, the time complexity of 2STEP attack will be $O(TN^2M)$, where $T\approx300$ is the game length, $N\approx150$ is the average action number for a state, and $M \geq 800$ is simulation count of the examiner. Hence, we need a more efficient algorithm.

{\color{red}(not clear what are the main contributions here to reduce the complexity. )}

\input{algorithm/basic}
Algorithm \ref{alg:basic} shows the algorithm of searching an value adversarial example. The input includes a sequence of states $s_i$ representing the game, a target agent $t$, and an examiner agent $e$ (line). Both target and examiner agent have a lookup-table to store the result they have evaluated before. For example, if we call $t.V(s)$ the first time, the examiner will evaluate state $s$ and return the value $V(s)$. Next, if we call $t.\pi(s)$, we can get the policy without evaluating $s$ again.  
The algorithm will loop through all the states $s_i$ in the game to find the existence of an example(line 2). For each $s_i$, we first check that if $s_i$ is too hard for the target (line 3). If so, we will skip this state (line 4). Next, we use the examiner to get the meaningless actions of state $s_i$ (line 6). The meaningless actions of the turn player store in $actions[0]$, other store in $stores[1]$. Line 7 to 9 gets the candidate state $s'$ by test all the combination of the meaningless actions. 
Since the computation of examiner is expensive, before we use it to evaluate $s'$, we first probe is $|t.v(s') - e.V(s)| \geq thr_{adv} - thr_{eq}$ (line 10), which is the necessary condition of $s'$ being an adversarial example (proof is in appendix). Since $b_0, b_1$ are meaningless actions, $s'$'s winrate is mostly the same as $s$ and the target agent can tell that. Hence, this step can filter out most of $s'$ (more than 97\% in our experiment).
Finally, in line 11 to 12, we check does $s'$ satisfy our criterion and return $s'$ if it is.
The algorithm of searching an policy example is basically changing the target agent's value $t.v$ in Algorithm \ref{alg:basic} to the action value $e.Q$ of the recommended action of target agent $\arg \max_{a}(p)$. (See appendix)


We improve the efficiency of getting the meaningless action, by proving the meaningful actions (actions that are not meaningless) of $s_t$ are mostly also the meaningful actions of $s_{t-1}$ (see appendix). The intuition is that as more stones are placed, meaningful actions will gradually become meaningless or illegal since more and more positions become one's territory. 
Therefore, by searching all the states reversely (line 3), once we verify an action is meaningful at state $s_t$, we do not need to verify it again on states $s_i, i < t$. 
Additionally, instead of directly using the examiner, we use the PV-NN of examiner to exam action first. If an action looks meaningful to PV-NN, we will use the examiner to verify that. 














==> backup.tex <==

\subsection{Problem Setup}



In this section, we will first define the criterion of both policy and value adversarial examples. Next we will talk about how to find such examples efficiently. 

\subsection{Problem Setup}
Our goal is to find adversarial examples of a "target" agent. The target can be a PV-NN or a PV-MCTS agent as long as it can provide the value $v(s)$ and the policy $p(s)$ for a given state $s$. 
However, since there is no ground truth in Go, we need a "examiner" agent to verify the output of the student agent. 
The examiner should be able to provide the value $V(s)$, the policy $\pi(s)$, and the action $Q(s,a)$ for a given state $s$. 
For example, the examiner we used is the strongest PV-MCTS agent we have. Note that the target can be the same PV-MCTS agent as long as the examiner has much more simulations. 

For an adversarial example $s'$ modified from a nature state $s$, we expect 1) $s'$ looks almost the same as $s$, 2) $s'$ is semantically the same as $s$, 3) the target agent is truly wrong, 4) humans can interpret that the target agent is wrong with only given the target output of $s, s'$.
The first three points are mimicking the adversarial examples in NLP. 
The forth point is to ensure the mistake is stupid enough that even human can verified it independently  without the help of examiner. In the following sections, we first limit the search space of our adversarial example. Next, we provide criterion for both value and policy adversarial example of student agent.


\subsubsection{Search space restriction}
\label{section:search_space}
To achieve the our expectation for adversarial examples, we first limit the search space with the examiner agent before testing any target agent. Given a state $s$, the search space $\mathcal{B}(s)  \subset \mathcal{S}$ of adversarial examples $s'$ is defined by the following three steps. 

First, to make the adversarial example $s_t'$ looks almost the same as $s_t$, the adversarial example should be at most two actions away from the original state $s_t$. Since each action will only add one stone on the board in Go, the board will looks almost the same. If we decompose the state $s_t'$'s trajectory to a list of actions, it will looks like $a_0, a_1, \dots, a_{t-1}, b_0, b_1$,
where $a_0, a_1, \dots, a_{t-1}$ is the trajectory of state $s_t$ and $b_0, b_1$ are the extra actions we add. 
Note that we cannot add only one action $b_0$ since it will change the turn player, which violate the second point of our expectation.
However, one of the $b_i$ can be a pass action $a_pass$. If one of the $b_i$ is a pass action, we call it \textbf{one-step attack}, since we only place one additional stone on the board.
Likewise, if both $b_i$ are not is a pass action, we call it \textbf{two-step attack} .
We do not include states that created by deleting or randomly adding actions to the trajectory of the state $s_t$. 
since such states can easily be illegal or change the circumstances of the game. We also do not include replacement. Unlike NLP can replace a word with its synonyms, there are no similar actions in Go. 

Second, we use the examiner agent to ensure $s'$ semantically be the same as $s$. 
The examiner, which is a PV-MCTS agent, is very sensitive to any changes. Even if one of the agents gets a small advantage, which is not enough to win the game, it will still reflect on its output winrate $V(s)$.  
Hence, we define that two states $s, s'$ is semantically the same if they have the same turn player $s.c = s'.c$ and a close enough winrate $|V(s)- V(s')| \leq thr_{eq}$, where $thr_{eq}$ is a small threshold that we can tolerate. 

Finally, to let human be able to understand the adversarial example, we require the actions new added should be \textbf{meaningless}. Even though we have restrict that the winrate $V(s), V(s')$ should be almost the same for the examiner. However, it doesn't means that humans can have the same judgement since humans are way weaker than the examiner. When game is too complicate, human can not tell who is wining and if an action is bad. 
Luckily, even though humans cannot understand high-end games, there exists meaningless actions that humans can tell that those actions do not help players get any more advantage with some simple domain knowledge of Go. For example, it is meaningless for a player to place a stone in a position he has already occupied.
By only adding such meaningless action, regular human players can certify that the situation is the same without knowing which color is winning.


{\color{red}(cho: discuss; how does this relate to human checkibility? )}
To automatically find meaningless actions that humans can certify, we again use the examiner's output value $V(s)$. For convenience, we define a function $free\_play(s, a): \mathcal{S} \times \mathcal{A} \mapsto \mathcal{S}$ as playing action $a$ on state $s$ without changing the turn player by skipping the opponent's turn. Since action's color $a.c$ might not be the turn color of $s$, $free\_play$ is formulated as follow:

\[ 
free\_play(s,a)=
\begin{cases} 
  \mathcal{T}(\mathcal{T}(s,a),a_{pass})  & s.c = a.c \\
  \mathcal{T}(\mathcal{T}(s,a_{pass}), a) & s.c \neq a.c
\end{cases}
\]

where $s.c, a.c$ are the color of the state and the action, $a_{pass}$ is the pass action. Finally, we find meaningless action $a$ by checking if $|V(s)-V(free\_play(s,a))|\leq thr_{eq}$, where $thr_{eq}$ is the same small threshold that we can tolerant. In intense games like Go, if one player play an extra action freely $V(free\_play(s,a))$, it is supposed to favorite the color $a.c$. Therefore, if the winrate $V((free\_play(s,a)))$ do not change, the action is likely to be meaningless to humans, which is mostly true according to our human study.

{\color{red}(cho: Did you mention territory? I think we are searching within the territory? )}

\subsubsection{Criterion of Adversarial Attack}

In the previous section, we limit the search space $\mathcal{B}$ with the examiner. In this section, we are going to define what kind of target agent's outputs should be for an adversarial example so that the example meet our expectations. Since the target agent has two outputs, the state value $v(s)$ and the policy $p(s)$, we will define criterion for each of them.

For the value output, we define $s'$ is the value adversarial example of $s$, if 
\begin{enumerate}
    \item $s' \in \mathcal{B}(s)$
    \item $|v(s)-V(s)| \leq thr_{correct}$
    \item $|v(s')-V(s')| \geq thr_{is\_adv}$
\end{enumerate}
The first point has been discussed in \ref{section:search_space}. The second point is to ensure that the target agent's value output is correct to the examiner before attack. $thr_{correct}$ is an acceptable threshold. If the target agent is not correct before attack, then it is no surprising that it will be wrong after attack, which is not we want.
The third point means that the target's output $v(s')$ is unacceptably wrong to the examiner. 
$thr_{is\_adv}$ is a threshold that define the error degree that can be define as an adversarial example. 
For example, if we want to find an example that PV-NN misclassified the winning color of a state, we can set $thr_{is\_adv}=0.5$. Since $v(s'),V(s') \in [0,1]$, every example that is $V(s') \geq 0.5$ will have a $v(s') \leq 0.5$. If we want the target's output $v(s)$ is not only wrong, but with high confidence with its answer, we can set $thr_{is\_adv}$ larger.

According to our human study, without the help of examiner ,humans are able to certify the target agent is wrong on the adversarial examples that satisfy above criterion. They normally shows target agent is wrong by following steps. First, they notice that winrate of $s$ and $s'$ should be the same since the additional actions are meaningless. Next, when they see that $v(s)$ is very different from $v(s')$, they immediately know that at least one of value outputs $v(s), v(s')$ is wrong.


For the policy output, define the criterion is even more challenging. Unlike normal classification, there is more than one best action for a state. Moreover, even the recommended action is genuinely incorrect, can a human player verify that? With these in mind, we define $s'$ as the policy adversarial example of $s$, if 
\begin{enumerate}
    \item $s' \in \mathcal{B}(s)$
    \item $|Q(s, a_s )-V(s)| \leq thr_{correct}$
    \item $|Q(s', a_{s'} )-V(s')| \geq thr_{is\_adv}$
    \item $|Q(s', a_s )-V(s')| \leq thr_{correct}$
    \item $|Q(s, a_{s'} )-V(s)| \geq thr_{is\_adv}$
\end{enumerate}
where $a_s = \arg \max_{a}(p(a|s))$ is the target agent's recommended action of state $s$ and $a_{s'} = \arg \max_{a}(p(a|s'))$ is the target agent's recommended action of state $s'$.
The first three points correspond to the three points of attacking value $v(s)$.
The first point is the same. The second point checks if the current state $s$ is too hard for target and cannot provide a proper action. The third point checks that is target malfunction and provides an action that has a very low action value for state $s'$. 

With the first three points, we have the adversarial example that can be understood by the examiner. However, humans still cannot verify if $ a_{s'}$ is a terrible chose. Luckily, in our human study, although action $a_{s'}$ may not look bad for humans, once we provide humans with $a_s$, they can immediately tell that $a_s$ is much more important to play than $a_{s'}$ in the state $s'$ and certify that the target agent is wrong. Hence, we add the fourth and fifth point to ensure that $a_{s}$ is a good action and $a_{s'}$ is a bad action for both $s, s'$, so that human player can use them as an anchor.

\input{algorithm}



==> pics/intro_pic.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=5cm]{pics/images/game.pdf}
% \vspace*{-3mm}
\caption{An adversarial example we found that can attack KataGo with 50 MCTS simulations. The example is perturbed from an AlphaGo Zero self-play record. Actions B19 and P1 (marked as 1 and 2) are the meaningless actions we add as the perturbation. In this state, the black player is supposed to play at position A to kill all the white stones marked with squares. However, confused by the actions we added, the agent ends up playing B to save the four black stones marked with triangles and gives up the opportunity to occupy way more territories by playing position A.
}
\label{fig:intro_pic}
\end{figure}

==> pics/k40vsk20.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
    width=10cm,
    height=8cm,
    mark options={solid},
    xlabel={KataGo 20 blocks simulation count},
    ylabel={Attack success rate},
    symbolic x coords={5, 25, 100, 400, 1600},
    xmin=5, xmax=1600,
    ymin=-0.1, ymax=1.2,
    enlarge x limits=0.05,
    xtick={5, 25, 100, 400, 1600},
    ytick={0, 0.25, 0.5, 0.75, 1.0},
    ymajorgrids=true,
    tick style={draw=none},
    grid,
    grid style={dotted,gray!70},
    legend style={font=\normalsize,legend pos=north west,cells={anchor=west},fill=gray!4},
    axis background/.style={fill=gray!3}
]
 
 \addplot [
    color=blue!45,
    line width=0.3mm,
    mark=diamond*,
    dashed
    ]
    coordinates {
    (5,0.35)(25,0.55)(100,0.55)(400,0.75)(1600,0.9)
    };
    \addlegendentry{value 1STEP}
 \addplot [
    color=blue,
    line width=0.3mm,
    mark=square*
    ]
    coordinates {
    (5,0.40)(25,0.55)(100,0.65)(400,1.00)(1600,1.00)

    };
    \addlegendentry{value 2STEP}

 

 \addplot [    
    color=red!45,
    mark=triangle*,
    line width=0.3mm,
    dashed
    ]
    coordinates {
    (5,0.00)(25,0.05)(100,0.18)(400,0.32)(1600,0.65)
    };
    \addlegendentry{policy 1STEP}

    
  \addplot [
    color=red,
    line width=0.3mm,
    mark=*,
    ]
    coordinates {
    (5,0.05)(25,0.23)(100,0.50)(400,0.82)(1600,0.9)
    };
    \addlegendentry{policy 2STEP}
  
    
\end{axis}
\end{tikzpicture}

\vspace*{-3mm}

\caption{The attack success rate of $\eta_\text{adv} = 0.7$ on datasets that are generated by KataGo 40 blocks with 800 simulations vs KataGo 20 blocks with different number of  simulations. }
\label{fig:k40vsk20}

\end{figure}

==> pics/policy_fail.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=6cm]{pics/images/policy_fail_az_game4.pdf}
\caption{policy fail}
\label{fig:policy_fail}
\end{figure}

==> pics/policy_succ.tex <==
% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm]{pics/examples/14k_1.sgf.tksk_p0.9.pdf}
% \caption{Policy success.}
% \label{fig:policy_succ}
% \end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\linewidth}        %% or \columnwidth
        \centering
        \includegraphics[width=\textwidth]{pics/examples/14k_1.sgf.tksk_p0.9.pdf}
% \caption{policy fail}
\label{fig:policy_fail}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\linewidth}        %% or \columnwidth
        \centering
        \includegraphics[width=\textwidth]{pics/examples/13k_1.sgf.tksk_v0.9.pdf}
% \caption{value fail}
\label{fig:value_fail}
    \end{subfigure}
    % \vspace*{-8mm}
    \caption{Adversarial example of policy attack (left) and value attack (right) on FOX.
    % \vspace{10pt}
    }
    \label{fig:succ}
\end{figure}

==> pics/value_fail.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=6cm]{pics/images/value_fail_atv_1.pdf}
\caption{value fail}
\label{fig:value_fail}
\end{figure}

==> pics/value_succ.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=6cm]{pics/examples/13k_1.sgf.tksk_v0.9.pdf}
\caption{value success}
\label{fig:value_succ}
\end{figure}

==> related.tex <==

Go AI. 
% We conduct experiments on four open-sourced programs, including KataGo \cite{wu2019accelerating}, ELF OpenGo \cite{tian2019elf}, Leela Zero \cite{LeelaZero}, and CGI \cite{wu2020accelerating}. For KataGo, we use 20 blocks and 40 blocks models. The 20 blocks model is released at 2020-11-28 21:22:13 UTC, and the 40 blocks model is released at 2021-08-11 10:15:42 UTC. For the remaining three programs, since they are no longer in development, we use their latest released models provided in their github project.

Adversarial examples in DNN. (Adversarial examples for computer vision, and some later works extended the attacks to discrete domain such as NLP, (how they are different from us). 

Some more discussions about attacks to RL agents and how they are different from us. 





==> tables/diff_agents.tex <==
\begin{table}[t]
\caption{Attack results on different agents with all datasets. ``EXECUTED NUM'' shows the average number of target and examiner calls for the attack, and ``SPEEDUP'' indicates the speedup of the proposed method over the brute-force search. }
\label{tab:diff_agents}
% \vskip 0.1in
\begin{center}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{sc}
\resizebox{.45\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{ccccccc}
\toprule
\multicolumn{2}{c}{} &  \multicolumn{2}{c}{success rate} & \multicolumn{2}{c}{executed num} & \\
\midrule
& {Agent} & {1step} & {2step} & {Target} & {Examiner} & {Speedup}\\
%   & \textbf{agent} & \textbf{1step} & \textbf{2step} & \textbf{target} & \textbf{examiner}\\
\midrule
% \multicolumn{7}{c}{ value attack with $\eta_{adv} = 0.5$} \\
\scriptsize \multirow{4}*{\shortstack[c]{Value \\ $\eta_{adv} = 0.5$}} 
& katago	& 0.99	& 1.00	& 6152	& 68  & 80 \\
& leela	& 0.90	& 0.98	& 37533	& 182  & 163\\
& elf	& 0.92	& 1.00	& 11108	& 108  &  90\\
& cgi	& 1.00	& 1.00	& 40	& 2   &  14 \\
\midrule[0.1pt]
% \multicolumn{7}{c}{ value attack with $\eta_{adv} = 0.7$} \\
\scriptsize \multirow{4}*{\shortstack[c]{Value \\ $\eta_{adv} = 0.7$}} 
& katago	& 0.86	& 0.94	& 44638	& 299 & 125 \\ 
& leela	& 0.70	& 0.84	& 96134	& 518     & 150 \\ 
& elf	& 0.65	& 0.87	& 42503	& 398     & 94  \\ 
& cgi	& 1.00	& 1.00	& 45	& 2       & 15  \\ 
\midrule[0.1pt]
% \multicolumn{7}{c}{ policy attack with $\eta_{adv} = 0.5$} \\
\scriptsize \multirow{4}*{\shortstack[c]{Policy \\ $\eta_{adv} = 0.5$}} 
& katago	& 0.70	& 0.92	& 128228 & 666 & 155\\ 
& leela	& 0.92	& 0.97	& 17218	& 118 & 123\\ 
& elf	& 0.93	& 0.97	& 16387	& 113 & 122\\ 
& cgi	& 0.87	& 0.96	& 16495	& 103 & 133\\ 
\midrule[0.1pt]


% \multicolumn{7}{c}{ Policy attack with $\eta_{adv} = 0.7$} \\
 \scriptsize \multirow{4}*{\shortstack[c]{Policy \\ $\eta_{adv} = 0.7$}} 
& katago	& 0.55	& 0.82	& 231895 & 707 & 232  \\ 
& leela	& 0.75	& 0.93	& 36438	& 150    & 186    \\ 
& elf	& 0.77	& 0.88	& 31258	& 159    & 157   \\ 
& cgi	& 0.75	& 0.89	& 24915	& 139    & 146   \\ 
\bottomrule
% \multicolumn{5}{|c|}{ Value attack with $thr_{adv} = 0.9$} \\
% \hline
% kataGo	& 0.56	& 0.62	& 275685	& 1584 \\ 
% \hline
% \multicolumn{5}{|c|}{ Policy attack with $thr_{adv} = 0.9$} \\
% \hline
% kataGo	& 0.32	& 0.48	& 434876	& 859 \\ 

\end{tabular}
}
\end{sc}
\end{center}
\vskip -0.1in
\end{table}

==> tables/diff_dataset.tex <==
\begin{table}[t]
\caption{Attack  results on different  datasets. ``EXECUTED NUM'' shows the average number of target and examiner calls for the attack. }
% \caption{Experiment of different dataset on all agents. ZZ is AlphaGo Zero training data, ZM is AlphaGo Zero vs AlphaGo Master, MH is AlphaGo Master vs Human champions, LG is the final games of LG Cup World Go Championship (2001-2020), ATV is the  final games of Asian TV Cup (2001-2020), and FOX is the amateur games from online platform Fox.}
\label{tab:diff_dataset}
% \vskip 0.1in
\begin{center}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{sc}
\resizebox{.41\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{cccccc}


\toprule
\multicolumn{2}{c}{} &  \multicolumn{2}{c}{success rate} & \multicolumn{2}{c}{executed num}\\
\midrule
 & {Games} & {1step} & {2step} & {Target} & {Examiner}\\
%  & \textbf{agent} & \textbf{1step} & \textbf{2step} & \textbf{target} & \textbf{examiner}\\
\midrule

% \midrule[0.1pt]
\scriptsize \multirow{6}*{\shortstack[c]{Value \\ $\eta_{adv} = 0.7$}} 
& zz	& 0.78	& 0.89		& 14691	& 316	\\ 
& zm	& 0.90	& 0.95		& 12977	& 197	\\ 
& mh	& 0.60	& 0.81		& 173844	& 663\\ 
& lg	& 0.85	& 0.95		& 12650	& 161	\\ 
& atv	& 0.88	& 0.95		& 14988	& 185	\\ 
& fox & 0.83	& 0.94		& 53792	& 213	 \\ 
\midrule[0.1pt]
% \multicolumn{5}{c}{ Policy attack with $thr_{adv} = 0.5$} \\
% \midrule[0.1pt]
\scriptsize \multirow{6}*{\shortstack[c]{Policy \\ $\eta_{adv} = 0.7$}} 
&  zz	& 0.57	& 0.82		& 33314	& 502 \\ 
&  zm	& 0.84	& 0.94		& 13374	& 178 \\ 
&  mh	& 0.51	& 0.80	    & 227202& 258 \\ 
&  lg	& 0.84	& 0.96		& 52055	& 274 \\ 
&  atv	& 0.75	& 0.88		& 79688	& 232 \\ 
&  fox	& 0.75	& 0.87	 & 141120	& 225 \\ 
% \midrule[0.1pt]
% \multicolumn{5}{c}{ Value attack with $thr_{adv} = 0.7$} \\
% \midrule
% \scriptsize \multirow{4}*{\shortstack[c]{Value \\ $\eta_{adv} = 0.7$}} 
% & sim 5 & 0.36 & 0.41 & 4507.50 & 150.00 \\ 
% & sim 25 & 0.55 & 0.55 & 10496.50 & 243.00 \\ 
% & sim 100 & 0.55 & 0.68 & 10095.50 & 318.50 \\ 
% & sim 400 & 0.73 & 1.00 & 23441.50 & 333.50 \\ 
% \midrule
% \multicolumn{5}{c}{ Policy attack with $thr_{adv} = 0.7$} \\
% \midrule[0.1pt]
%  \scriptsize \multirow{4}*{\shortstack[c]{Policy \\ $\eta_{adv} = 0.7$}} 
% & sim 5 & 0.00 & 0.05 & 12287.50 & 244.00 \\ 
% & sim 25 & 0.05 & 0.23 & 77043.50 & 657.50 \\ 
% & sim 100 & 0.18 & 0.50 & 50516.00 & 792.50 \\ 
% & sim 400 & 0.32 & 0.82 & 55932.00 & 998.00 \\ 
\bottomrule
% \multicolumn{5}{|c|}{ Value attack with $thr_{adv} = 0.9$} \\
% \hline
% kataGo	& 0.56	& 0.62	& 275685	& 1584 \\ 
% \hline
% \multicolumn{5}{|c|}{ Policy attack with $thr_{adv} = 0.9$} \\
% \hline
% kataGo	& 0.32	& 0.48	& 434876	& 859 \\ 

\end{tabular}
}
\end{sc}
\end{center}
\vskip -0.1in
\end{table}





% \begin{table}[t]
% \caption{Experiment of different dataset on all agents}
% \label{tab:diff_dataset}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{  c  c  c  c   c }
% \toprule
% dataset & 1step & 2step & target & examiner\\



% \midrule
% \multicolumn{5}{c}{ value attack with $thr_{adv} = 0.7$} \\
% \midrule
% ZZ	& 0.78	& 0.89		& 14691	& 316	\\ 
% ZM	& 0.90	& 0.95		& 12977	& 197	\\ 
% MH	& 0.60	& 0.81		& 173844	& 663\\ 
% LG	& 0.85	& 0.95		& 12650	& 161	\\ 
% ATV	& 0.88	& 0.95		& 14988	& 185	\\ 
% FOX & 0.83	& 0.94		& 53792	& 213	 \\ 
% \midrule
% \multicolumn{5}{c}{ policy attack with $thr_{adv} = 0.7$} \\
% \midrule
% ZZ	& 0.57	& 0.82		& 33314	& 502 \\ 
% ZM	& 0.84	& 0.94		& 13374	& 178 \\ 
% MH	& 0.51	& 0.80	    & 227202& 258 \\ 
% LG	& 0.84	& 0.96		& 52055	& 274 \\ 
% ATV	& 0.75	& 0.88		& 79688	& 232 \\ 
% FOX 	& 0.75	& 0.87	 & 141120	& 225 \\ 
% \midrule
% \multicolumn{5}{c}{ value attack with $thr_{adv} = 0.7$} \\
% \midrule
% sim 5 & 0.36 & 0.41 & 4507.50 & 150.00 \\ 
% sim 25 & 0.55 & 0.55 & 10496.50 & 243.00 \\ 
% sim 100 & 0.55 & 0.68 & 10095.50 & 318.50 \\ 
% sim 400 & 0.73 & 1.00 & 23441.50 & 333.50 \\ 
% \midrule
% \multicolumn{5}{c}{ policy attack with $thr_{adv} = 0.7$} \\
% \midrule
% sim 5 & 0.00 & 0.05 & 12287.50 & 244.00 \\ 
% sim 25 & 0.05 & 0.23 & 77043.50 & 657.50 \\ 
% sim 100 & 0.18 & 0.50 & 50516.00 & 792.50 \\ 
% sim 400 & 0.32 & 0.82 & 55932.00 & 998.00 \\ 

% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

==> tables/mcts_different_simulations.tex <==
\begin{table}[t]
\caption{KataGo with different simulations on ZZ dataset. ``EXECUTED NUM'' shows the average number of target and examiner calls for the attack.}
\label{tab:mcts}
\vskip 0.1in
\begin{center}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{sc}
\resizebox{.38\textwidth}{!}{% <------ Don't forget this %

\begin{tabular}{cccccc}
\toprule
\multicolumn{2}{c}{} &  \multicolumn{2}{c}{success rate} & \multicolumn{2}{c}{executed num}\\
\midrule
 & {Sim} & {1step} & {2step} & {Target} & {Examiner}\\

\midrule
\scriptsize \multirow{6}*{\shortstack[c]{Value \\ $\eta_{adv} = 0.5$}} 
& 1  & 1.00 & 1.00 & 1016  & 41    \\
& 5  & 0.89 & 0.95 & 4454  & 2322  \\ 
& 10 & 0.89 & 0.95 & 6501  & 3147  \\
& 25 & 0.84 & 0.89 & 18516 & 13903 \\
& 50 & 0.53 & 0.58 & 76426 & 42974 \\

\midrule[0.1pt]
\scriptsize \multirow{6}*{\shortstack[c]{Policy \\ $\eta_{adv} = 0.5$}} 
& 1  & 0.84 & 1.00 & 18347 & 869    \\
& 5  & 1.00 & 1.00 & 3309  & 1318 \\
& 10 & 0.95 & 1.00 & 6666  & 2662 \\
& 25 & 0.79 & 1.00 & 12466 & 5487 \\
& 50 & 0.21 & 0.68 & 89512 & 41702 \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{center}
\vskip -0.1in
\end{table}

